Extended Abstract: Partial-encapsulate and Its Support for Floating-point Operations in ACL2

We illustrate the power of partial-encapsulate, showing how it is used in the implementation of floating-point operations in ACL2.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.6}{10.4204/EPTCS.423.6}}

